Unsupervised Deformable Image Registration for Respiratory Motion Compensation in Ultrasound Images

In this paper, we present a novel deep-learning model for deformable registration of ultrasound images and an unsupervised approach to training this model. Our network employs recurrent all-pairs field transforms (RAFT) and a spatial transformer network (STN) to generate displacement fields at online rates (apprx. 30 Hz) and accurately track pixel movement. We call our approach unsupervised recurrent all-pairs field transforms (U-RAFT). In this work, we use U-RAFT to track pixels in a sequence of ultrasound images to cancel out respiratory motion in lung ultrasound images. We demonstrate our method on in-vivo porcine lung videos. We show a reduction of 76% in average pixel movement in the porcine dataset using respiratory motion compensation strategy. We believe U-RAFT is a promising tool for compensating different kinds of motions like respiration and heartbeat in ultrasound images of deformable tissue.

==> quick_links.tex <==
1. Drive folder:
https://drive.google.com/drive/folders/15s4Qm8A6ddYwYheuPLQHfa1QKq-EgYxZ?usp=sharing

2. Diagram ppt:
https://docs.google.com/presentation/d/1OE0OuoI7Q8jwBvB_15eEBkHA76ipYBjY_qxMT1PPr64/edit?usp=sharing
